Closed-form solutions for the Salpeter equation

We propose integral representations and analytical solutions for the propagator of the $1+1$ dimensional Salpeter Hamiltonian, describing a relativistic quantum particle with no spin. We explore the exact Green function and an exact solution for a given initial condition, and also find the asymptotic solutions in some limiting cases. The analytical extension of the Hamiltonian in the complex plane allows us to formulate the equivalent stochastic problem, namely the B\"aumer equation. This equation describes \textit{relativistic} stochastic processes with time-changing anomalous diffusion. This B\"aumer propagator corresponds to the Green function of a relativistic diffusion process that interpolates between Cauchy distributions for small times and Gaussian diffusion for large times, providing a framework for stochastic processes where anomalous diffusion is time-dependent.

==> src/02_General_Formalism.tex <==
\section{General Formalism}\label{sec:GeneralFormalism}



==> src/04_Asymptotic_sol.tex <==
\section{Asymptotic Solutions}~\label{SEC:Asymp}

\Blue{we need the asymptotic solutions resulting from the asymptotic behavior of the modified Bessel function for small/large arguments. We need to write the equations of this assymptotic behavior and a reference.}




\subsection{Case \texorpdfstring{$x \to t$}{x  t}}
When $x \to t^+$, which means the particle is approaching the light cone from the right side, the asymptotic solution follows the modified Bessel function (See Eq.~\ref{Eq:asymptotic} in Appendix~\ref{app:differential})
%
\begin{equation}
    K_1(y)\to \frac{1}{y}+ \frac{y}{2}\ln \frac{y}{2} + O(y), \ \ y\to 0
\end{equation}
where $y=mr, r=\sqrt{x^2+\tau^2}$, and $\tau=it$.

When $x \to t^-$, indicating that the particle approaches the light cone from the left side, the asymptotic solution is for the Hankel function. We calculate by substituting $y$ with $iy$, thus $iy=im\sqrt{x^2-t^2}$. Utilizing the relationship between the modified Bessel function and Hankel function (Eq.~\ref{eq:B_to_H}), we have:
\begin{equation}
    K_1(y) = -\frac{\pi}{2} H_1^{(1)}(iy)
\end{equation}
Thus the asymptotic solution for $x \to t^-$ is:
\begin{equation}
    H_1^{(1)}(y) \to -\frac{\pi}{2iy}- \frac{\pi i y}{4}\ln \frac{y}{2}+O(y), \ \ y\to 0 
\end{equation}



==> src/appx5_case.tex <==
\section{Case \texorpdfstring{$mt\gg 1$}{mt 1}}
The explicit form of the functions has been shown in SEC.~\ref{app:scaling}. Especially, for the case $mt\gg 1$, a generic $mx$ we obtain

\begin{equation}
\begin{split}
\left. G\right|_{mt\gg 1}\to & m\sum_{n=0}^{\infty}\frac{A_n^{(1)}(mt)^n}{(2n)!}f_n(mx)\\
&+\frac{m}{2}\sum_{s=\pm}\sum_{n=0}^{\infty}\frac{(-i)^n(mt)^n}{2^nn!}\text{Ei}_n\left[im(t-sx)\right]
\end{split}
\end{equation}
The second term can be re-summed easily to obtain
\begin{equation}
\begin{split}
&\sum_{n=0}^{\infty}\frac{(-i)^n(mt)^n}{2^nn!}\text{Ei}_n(im(t-sx))\\
&=\int_1^{\infty}e^{-im(t-sx)z-\frac{imt}{2z}}\text{d}z
\end{split}
\end{equation}
For the small and large $mx$ values, we can use Eqs.~\ref{Eq:smallf} and~\ref{Eq:largef} respectively. For the small $mx$ and large $mt$ values we have ($O\left[(\frac{x}{t})^2\right]$)
\begin{equation}
\begin{split}
\left. G\right|_{mt\gg 1,mx\ll 1}\to & m\sum_{n=0}^{\infty}\frac{A_n^{(1)}(mt)^n}{(2n)!}\left(\frac{1}{2n+1}-\frac{m^2x^2}{2(2n+3)}\right)\\
&+m\int_1^{\infty}e^{-imt(z-\frac{1}{2z})}\text{d}z
\end{split}
\end{equation}
while for the large $mx$ (and again large $mt$) values one finds
\begin{equation}
\begin{split}
\left. G\right|_{mt\gg 1,mx\gg 1}\to & \left(\sum_{n=0}^{\infty}\frac{A_n^{(1)}(mt)^n}{(2n)!}\right)\frac{\sin mx}{x}\\
&+\frac{m}{2}\sum_{s=\pm}\int_1^{\infty}e^{-im(t-sx)z-\frac{imt}{2z}}\text{d}z
\end{split}
\end{equation}

%This isthe amaysing table
\renewcommand{\arraystretch}{2.3}

\begin{table*}[h]
\centering
\begin{tabular}{ |P{0.15cm}|P{1.5cm}|P{3.05cm}|P{6.45cm}|P{2.9cm}|P{2cm}| } 
\hline
N & Model & Hamiltonian $H(p)$ & 
$\phi_\pm(x,t,\rho,\theta)=\Re{-iH(\rho e^{i\theta})}t\pm \rho x \sin{\theta}$ & $\phi_+\to -\infty$ & Authors \\
\hline
1 & Relativistic quantum mechanics & $(p^2c^2+m^2c^4)^{1/2}$ 

& $\begin{aligned} &\Re{-i(\rho^2 c^2 e^{2i\theta}+m^2c^4)^{1/2} t} \pm \rho \sin{\theta} x\\
                   & \sim -\rho(-ct\pm x)\sin{\theta} \end{aligned}$ 


&if $x<ct$, $D_4$ for $G_+$ and $D_2$ for $G_-$ & Salpeter \cite{kowalski2011salpeter},    \\ 
\hline
2 & Relativistic stochastic mechanics & $-i(p^2c^2+m^2c^4)^{1/2}$ 

& $\begin{aligned} &\Re{-(\rho^2 c^2 e^{2i\theta}+m^2c^4)^{1/2}} \pm \rho \sin{\theta} x\\
                   & \sim -\rho(ct \cos{\theta} \pm x\sin{\theta}) \end{aligned}$ 

& $D_1$ for $G_+$ and $D_4$ for $G_-$ & Andreu et al. \cite{andreu2007some},  Beeumer et al. \cite{baeumer2010stochastic}  \\ 
\hline
3 & Fractional quantum mechanics & $Dp^\alpha$ 

& $\begin{aligned} &\Re{-i\rho^\alpha e^{i\alpha\theta}D} \pm \rho \sin{\theta} x\\
                   & = -\rho(-Dt \cos{\theta} \pm x\sin{\theta}) \end{aligned}$ 

& $D_1$ for $G_+$ & Laskin \cite{Laskin2020fractional},    \\ 
\hline
\hline
3 & Fractional stochastic mechanics & $-iD p^\alpha$ 

& $\begin{aligned} &\Re{-\rho^\alpha e^{i\alpha\theta}D^\alpha} \pm \rho \sin{\theta} x\\
                   & = -\rho(-Dt \cos{\theta} \pm x\sin{\theta}) \end{aligned}$ 

& $D_1$ for $G_+$ & Levy \cite{arias2018closed},    \\ 
\hline
\end{tabular}
\caption{Summary of the FPMEs and their Green functions. Equations marked with (*) are used to fit the PDF  of the S\&P500 index, while ($\star$) represents the best model. }

\label{table:1}
\end{table*}
{\color{red}This part is extra, please move it to another place, or remove $\to$}
We will apply the theorem to the propagator in Eqs \ref{eq:propagator_pm} in this case 
\begin{equation}
    \Phi_\pm(p) = -iH(p)t\pm ipx
    \label{eq:Phi_Hamiltonian}
\end{equation}
Thus, we define the following function
\begin{equation}
\begin{split}
    &\phi_\pm(x,t,\rho,\theta)=\Re{\Phi_\pm(\rho e^{i\theta})}\\
    &=\Re{-iH(\rho e^{i\theta})}t\mp \rho x \sin{\theta})
\end{split}
\end{equation}
The condition \ref{eq:condition_4} reduces to 
\begin{equation}
    \lim_{\rho\to\infty}{\phi_\pm(x,t,\rho,\theta)}= -\infty
\end{equation}
and we find out the quadrant where the condition is satisfied.


==> src/appx7_probabilityConservation.tex <==
\section{Theorem of Residues}
\label{app:theoremofResidues}

